From Small-World Networks to Comparison-Based Search

The problem of content search through comparisons has recently received considerable attention. In short, a user searching for a target object navigates through a database in the following manner: the user is asked to select the object most similar to her target from a small list of objects. A new object list is then presented to the user based on her earlier selection. This process is repeated until the target is included in the list presented, at which point the search terminates. This problem is known to be strongly related to the small-world network design problem. However, contrary to prior work, which focuses on cases where objects in the database are equally popular, we consider here the case where the demand for objects may be heterogeneous. We show that, under heterogeneous demand, the small-world network design problem is NP-hard. Given the above negative result, we propose a novel mechanism for small-world design and provide an upper bound on its performance under heterogeneous demand. The above mechanism has a natural equivalent in the context of content search through comparisons, and we establish both an upper bound and a lower bound for the performance of this mechanism. These bounds are intuitively appealing, as they depend on the entropy of the demand as well as its doubling constant, a quantity capturing the topology of the set of target objects. They also illustrate interesting connections between comparison-based search to classic results from information theory. Finally, we propose an adaptive learning algorithm for content search that meets the performance guarantees achieved by the above mechanisms.

==> hardness.tex <==
We begin our proof by first proving that the randomized version of \textsc{SWND} is no harder than its deterministic version. We will use the following lemma
\begin{lemma}[Gummadi \cite{gummadi}]\label{ramki}
For any random variable $\mathcal{S}\subset \Nn$ that satisfies $|\mathcal{S}|\leq \beta$, there exists a deterministic set $\myset{S}^*$ s.t. $|\myset{S}^*|\leq \beta$ and
$$\bar{C}_{\myset{S}^*}\leq \bar{C}_{\myset{S}}$$
\end{lemma}
\begin{proof}
Observe that
\begin{align*} \bar{C}_{\myset{S}} &= \sum_{(s,t)\in \Nn\times\Nn}\lambda(s,t)\expect[C_{\myset{S}}(s,t)] \\&= \sum_{(s,t)\in \Nn\times\Nn}\!\!\!\lambda(s,t)\!\!\!\sum_{S\subset\Nn\times \Nn: |S|\leq \beta}\!\!\!\!C_{S}(s,t)\prob(\myset{S} = S)\geq  \bar{C}_{S^*}(s,t) \end{align*}
where $S^*=\arg\min C_{S}(s,t)$.\end{proof}

Define $\textsc{DetSWND}$ to be the same as \textsc{SWND} with the additional restriction that $\myset{S}$ is deterministic. 
Lemma~\ref{ramki} has the the following immediate implication.
\begin{corollary} The problem \textsc{SWND}($\Nn$,$\myset{M}$,$d$,$\mathcal{L}$,$\lambda$) is equivalent \textsc{DetSWND}($\Nn$,$\myset{M}$,$d$,$\mathcal{L}$,$\lambda$). In particular, any optimal solution of \textsc{DetSWND}($\Nn$,$\myset{M}$,$d$,$\mathcal{L}$,$\lambda$) will also be an optimal solution of  \textsc{SWND}($\Nn$,$\myset{M}$,$d$,$\mathcal{L}$,$\lambda$). Moreover, given a solution $\mathcal{S}$ of \textsc{SWND}($\Nn$,$\myset{M}$,$d$,$\mathcal{L}$,$\lambda$), any deterministic $S$ belonging to the support of $\mathcal{S}$ will be an optimal solution of \textsc{DetSWND}.
\end{corollary}
%\begin{quote}
%\textsc{Deterministic Small-World Network Design (DetSWND)}:
%Given $\myset{L}$, a demand distribution $\lambda$, and an integer $\beta>0$, select minimize 
%$$\bar{C}_{\myset{S}}= \sum_{(s,t)\in \Nn\times\Nn}\lambda(i,j)C_{\myset{S}}(i,j)$$ subject to $|\myset{S}|\leq\beta$.
%\end{quote}

As a result, to show that \textsc{SWND} is NP-hard, it suffices to show that \textsc{DetSWND} is NP-hard.
The latter is equivalent to the following problem.
\begin{quote}
\textsc{Weighted Deterministic Small-World Network Design  (W-DetSWND)}:
Given an embedding of $\Nn$ into $(\myset{M},d)$, a set of local edges $\myset{L}$,  a non-negative weight function $w$, and an integer $\beta>0$,
 minimize 
$$\bar{C}_{\mathcal{S}}^w=\sum_{(s,t)\times \Nn\times\Nn}w(s,t)C_{\mathcal{S}}(s,t)$$
subject to $|S|\leq\beta$. \end{quote}
The difference from  \textsc{DetSWND} is that
$w\geq 0$ may be any non-negative weight function and need not sum up to one. %: we require that $\sum_{(s,t)\times \Nn\times\Nn}w(s,t)>0$ but the above quantity may not necessarily be equal to one.

We call $\bar{C}_{\mathcal{S}}^w$ the weighted forwarding cost.
The equivalence of the two problems is implied by the fact that instance of \textsc{DetSWND} is also an instance of \textsc{W-DetSWND} (trivially), and any instance of  \textsc{W-DetSWND}
can be converted to an instance of \textsc{DetSWND} by setting $$\lambda(i,j) = \frac{w(i,j)}{\sum_{(s,t)\times \Nn\times\Nn}w(s,t)},\quad \text{for every pair}~(i,j).$$

We therefore turn our attention on \textsc{W-DetSWND}. 

\begin{theorem} \textsc{W-DetSWND} is NP-hard.
\end{theorem}
We show this by proving that the corresponding decision problem is NP-complete.
In particular, the decision problem  corresponding to  \textsc{W-DetSWND} is as follows
\begin{quote}
\textsc{W-DetSWND-D}: 
Given an embedding of $\Nn$ into $(\myset{M},d)$, a set of local edges $\myset{L}$,  a non-negative weight function $w$, and two constants $\alpha>0$ and $\beta>0$,
 is there a directed edge set $S$ such that $|S|\leq\beta$ and $$\sum_{(s,t)\times \Nn\times\Nn}w(s,t)C_{\mathcal{S}}(s,t)\leq\alpha?$$
\end{quote}
Note that, given the set of shorcut edges $S$, forwarding a message with greedy forwarding from any $s$ to $t$ can take place in polynomial time. As a result, \textsc{W-DetSWND-D} is in NP: given $S$, it can be verified within polynomial time (in $|\Nn|$) whether the weighted forwarding distance is less than or equal to $\alpha$.
We will prove it is also NP-hard by reducing the following NP-complete problem to it:
\begin{quote}
\textsc{VertexCover}: Given a graph $G(V,E)$ and a constant $k$, is there a set $A\subseteq V$ such that $|A|\leq k$ and $\Gamma(A)\cup A=V$, where $\Gamma(A)$ the neighborhood of $A$ in $G$?
\end{quote}

Given an instance $(G(V,E),k)$ of \textsc{VertexCover}, we construct an instance of  \textsc{W-DetSWND-D} as follows.
The set $\Nn$ in this instance will be embedded in a 2-dimensional grid, and the distance metric $d$ will be the Manhattan distance on the grid. In particular, let $n=|V|$ be the size of the graph $G$ and, w.l.o.g., assume that $V=\{1,2,\ldots,n\}$. Let 
\begin{align}
\ell_0&= 6n+3,\label{l0}\\
\ell_1&= n\ell_0+2= 6n^2+3n+2,\label{l1}\\
\ell_2&= \ell_1+3n +1= 6n^2+6n+3,\label{l2}\\
\ell_3&= 6n+3.\label{l3}
\end{align}
 We construct a $n_1\times n_2$ grid, where $n_1 = (n-1)\cdot \ell_0 +1$ and $n_2=\ell_1+\ell_2+\ell_3+1$. That is, the total number of nodes in the grid is $$N = [(n-1)\cdot \ell_0 +1]\cdot (\ell_1+\ell_2+\ell_3+1)=\Theta(n^4).$$
The object set $\Nn$ will be the set of nodes in the above grid, and the metric space will be $(\mathbbm{Z}^2,d)$ where $d$ is the Manhattan distance on $\mathbbm{Z}^2$. The local edges $\myset{L}$ is defined according to \eqref{local} with $r=1$, \emph{i.e.},
\begin{align}\myset{L}=\{(x,y)\in \Nn\times\Nn \text{ s.t. }d(x,y)\leq 1\}\label{localgrid}\end{align}
and any two adjacent nodes in the grid are connected by an edge in $\myset{L}$.

We now describe the weight function $w$.
Denote by $a_i$, $i=1,\ldots,n$, the node on the first column of the grid that resides at row $(i-1)\ell_0+1$. Similarly, denote by $b_i$, $c_i$ and $d_i$  the nodes on the columns $(\ell_1+1)$, $(\ell_1+\ell_2+1)$ and $(\ell_1+\ell_2+\ell_3+1)$  the grid, respectively, that reside at the same row as $a_i$, $i=1,\ldots,n$. These nodes are depicted in Figure~\ref{graph}.


 
\begin{figure}[t]
\begin{center}
\input{graph}
\end{center}
\caption{ A reduction of an instance of \textsc{VertexCover} to an instance of \textsc{W-DetSWND-D}. Only the nodes on the grid that have non-zero incoming or outgoing demands (weights) are depicted. The dashed arrows depict $A_1$, the set of pairs that receive a weight $W_1$. The solid arrows depict $A_2$, the set of pairs that receive weight $W_2$.}\label{graph}
\end{figure}


We define the weight  function $w(i,j)$ over the pairs of nodes in the grid as follows. To begin with, the pairs of grid nodes that receive a non-zero weight are the ones belonging to one of the following the sets:
\begin{align*}
A_1 &= \{(a_i,b_i)\mid i\in V\}\\
A_2 &= \{(b_i,b_j)\mid (i,j)\in E \}\!\cup\! \{(c_i,d_j)\mid (i,j)\in E\}\!\cup\!\{(c_i,d_i)\mid i\in V\}\\
A_3 &= \{(a_i,d_i)\mid i\in V\}
\end{align*} 
The sets $A_1$ and $A_2$ are depicted in Fig.~\ref{graph} with dashed and solid lines, respectively. Note that 
$$|A_1|= n$$ as it contains one pair for each vertex in $V$, $$|A_2|=4|E|+n$$ as it contains four pairs for each edge in $E$ and one pair for each vertex in $V$, and, finally, $$|A_3| = n.$$
The pairs in $A_1$ receive a weight equal to 
$$W_1 = 1,$$ the pairs in $A_2$ receive a weight equal to $$W_2 = 3n+1$$ and the pairs in $A_3$ receive a weight equal to
$$ W_3=1.$$
\begin{comment}
 In more detail:
\begin{itemize}
\item{\bf Pairs in $A_1$.}
For every $i\in V$, each pair $(a_i,b_i)$ is given a weight equal to $W_1$, \emph{i.e.},
$$w(a_i,b_i) = W_1, \qquad i=1,\ldots,n. $$
\item{\bf Pairs in $A_2$.}
For every edge $(i,j)\in E$ of the graph $G(V,E)$, the pairs $(b_i,b_j)$ and $(b_j,b_i)$ are given a weight equal to $W_2$, \emph{i.e.},
$$\text{for all }i,j\in V,\text{ if  }(i,j)\in E\text{ then }w(b_i,b_j)=w(b_j,b_i) = W_2.$$
Similarly, for every edge  $(i,j)\in E$ of the graph $G(V,E)$, the pairs $(c_i,d_j)$ and $(c_j,d_i)$ are also given a weight equal to $W_2$, \emph{i.e.},
$$\text{for all }i,j\in V,\text{ if  }(i,j)\in E\text{ then }w(c_i,d_j)=w(c_j,d_i) = W_2.$$
Moreover, for every $i\in V$, each pair $(c_i,d_i)$ is also given a weight equal to $W_2$, \emph{i.e.},
$$w(c_i,d_i) = W_2, \qquad i=1,\ldots,n. $$
\item{\bf Pairs in $A_3$. }For every $i\in V$, each pair $(a_i,d_i)$ is given a weight equal to $W_3$, 
\emph{i.e.},
$$w(a_i,b_i) = W_1, \qquad i=1,\ldots,n. $$
\item{\bf Remaining pairs.} All the remaining pairs receive a zero weight.
\end{itemize}
\end{comment}

For the bounds $\alpha$ and $\beta$ take
\begin{align}\alpha = 2W_1|A_1| + W_2\cdot |A_2| +3|A_3|W_3= (3n+1)(4|E|+n)+5n\label{alpha}\end{align}
and
\begin{align}\label{beta}\beta = |A_2|+n+k = 4|E|+2n+k.\end{align}

The above construction can take place in polynomial time in terms of $n$. It is easy to show that, if the graph $G$ has a vertex cover of size no more than $k$, one can construct a deterministic set of shortcut edges $\myset{S}$ that satisfies the constraints of \textsc{W-DetSWND-D}.

\begin{lemma} If the instance of \textsc{VertexCover} is a ``yes'' instance, then the constructed instance of \textsc{W-DetSWND-D} is also a ``yes'' instance. 
\end{lemma}

\begin{proof}

Suppose that there exists a vertex cover $A$ of the graph with size $|A|\leq k$. By the definition of $A$, for every $i\in V\setminus A$, there exists a $j\in A$ such that $i\in \Gamma(j)$, \emph{i.e.}, $i$ is a neighbor of $j$. We construct $\myset{S}$ as follows.
\begin{enumerate}
\item For every $i \in A$, add the  edges $(a_i,b_i)$ and $(b_i,c_i)$  in $\myset{S}$.
\item For every $i \in V\setminus A$, add an edge $(a_i,b_j)$ in $\myset{S}$, where $j$ is such that $j\in A$ and  $i\in\Gamma(j)$.
\item For every pair in $A_2$, add this edge in $\myset{S}$.
\end{enumerate}

\begin{figure}[t]
\begin{center}
\input{instance}
\end{center}
\caption{ A ``yes'' instance of \textsc{VertexCover} and the corresponding ``yes'' instance of \textsc{W-DetSWND-D}. The graph on the left is can be covered by two nodes, 1 and 4. The corresponding set $\myset{S}$ of shortcut contacts that satisfies the constraints of  \textsc{W-DetSWND-D} is depicted on the right.}\label{instance}
\end{figure}


The size of $\myset{S}$ is 
$$|\myset{S}| = 2|A|+(|V|-|A|)+ |A_2| = |A|+n+4|E|+n\leq 4|E|+2n+k.$$
Moreover, the weighted forwarding distance is
\begin{align*}
\bar{C}_{\mathcal{S}}^w& = \sum_{(i,j)\in A_1}W_1 C_{\mathcal{S}}(i,j) +\sum_{(i,j)\in A_2}W_2 C_{\mathcal{S}}(i,j) +\\
&\quad \sum_{(i,j)\in A_3}W_3 C_{\mathcal{S}}(i,j).
\end{align*}
We have
\begin{align}\sum_{(i,j)\in A_2}W_2 C_{\mathcal{S}}(i,j) = W_2 |A_2|\label{s1}\end{align}
as every pair in $A_2$ is connected by an edge in $\myset{S}$.



Consider now a pair  belonging to $A_1$, of the form $(a_i,b_i)$, $i\in V$. There is exactly one edge in $\myset{S}$ departing from $a_i$ which has the form $(a_i,b_j)$, where where either $j=i$ is or $j$ a neighbor of $i$. The distance of the closest local neighbor of $a_i$ from $b_i$ is $\ell_1-1$. The distance of $b_j$ from $b_i$ is at most $n\cdot \ell_0$. As
$$\ell_1-1=n\ell_0+2-1>n\ell_0 $$ 
the greedy forwarding will follow the edge $(a_i,b_j)$. If $b_j=b_i$, then $C_{\mathcal{S}}(a_i,b_i)=1$. If $b_j\neq b_i$, as $j$ is a neighbor of $i$, $\myset{S}$ contains the edge $(b_j,b_i)$. Hence, if $b_j\neq b_i$, $C_{\mathcal{S}}(a_i,b_i)=2$. As $i$ was arbitrary, we get that 
\begin{align}\sum_{(i,j)\in A_1}W_1 C_{\mathcal{S}}(i,j)\leq 2W_1n.\label{s2} \end{align}

Next, consider a pair in $A_3$ of the form $(a_i,d_i)$. For the same reasons as for the pair $(a_i,b_i)$, the shortcut edge $(a_i,b_j)$ in $\myset{S}$ will be used by the greedy forwarding  algorithm. In particular, the distance of the closest local  neighbor of $a_i$ from $d_i$ is $\ell_1+\ell_2+\ell_3-1$. The distance of $b_j$ from $d_i$ is at most $\ell_2+\ell_3+n\cdot\ell_0$. 
 As $\ell_1-1>n\ell_0 $,
the greedy forwarding will follow the edge $(a_i,b_j)$. 

By the construction of $\myset{S}$, $b_j$ is such that $j\in A$. As a result, again by the construction of $\myset{S}$, $(b_j,c_j)\in \myset{S}$. The closest local neighbor of $b_j$ to $d_i$ has  $\ell_2+\ell_3+d(b_j,b_i)-1$ Manhattan distance from $d_j$. Any shortcut neighbor $b_k$ of $b_j$ has at least $\ell_2+\ell_3$ Manhattan distance from $b_i$. On the other hand, $c_j$ has $\ell_3+d(b_j,b_i)$ Manhattan distance from $d_i$. As 
$\ell_2>1$ and $\ell_2>n\ell_0\geq d(b_j,b_i)$, the greedy forwarding algorithm will follow $(b_j,c_j)$. Finally, as $A_2\subset \myset{S}$, and $j=i$ or $j$ is a neighbor of $i$, the edge $(c_j,d_i)$ will be in $\myset{S}$. Hence, the greedy forwarding algorithm will reach $d_j$ in exactly 3 steps. As $i\in V$ was arbitrary, we get that
\begin{align}\sum_{(i,j)\in A_3}W_3 C_{\mathcal{S}}(i,j)= 3W_3n.\label{s3} \end{align}
From \eqref{s1},\eqref{s2}, and \eqref{s3} we get that 
\begin{align*} \bar{C}_{\mathcal{S}}^w& \leq 2W_1n+ W_2 |A_2|+ 3W_3n = \alpha
\end{align*}
and, therefore, the instance of \textsc{W-DetSWND-D} is also a ``yes'' instance.
\end{proof}

To complete the proof, we show that a vertex cover of size $k$ exists only if there exists a $\myset{S}$ that satisfies the constraints in constucted  instance of \textsc{W-DetSWND-D}.

\begin{lemma}
 If the constucted  instance of \textsc{W-DetSWND-D} is a ``yes'' instance, then the  instance of \textsc{VertexCover} is also a ``yes'' instance. 
\end{lemma}
\begin{proof}
\sloppy Assume that the constucted  instance of \textsc{W-DetSWND-D} is a ``yes'' instance, \emph{i.e.}, there exists a set $\myset{S}$, with $|\myset{S}|\leq \beta$  such that the augmented graph has a weighted forwarding distance less than or equal to $\alpha$.

\fussy
\begin{lemma} \label{lemmaS2}$A_2\subseteq \myset{S}$, \emph{i.e.}, the set $\myset{S}$ will contain all edges in $A_2$.
\end{lemma}
\begin{proof}Suppose that it does not. Then, there is at least one pair of nodes $(i,j)$ in $A_2$ with $C_{\mathcal{S}}(i,j)\geq 2$. Therefore, the weighted forwarding distance is 
\begin{align*}\bar{C}_{\myset{S}}^w&\geq 1\cdot W_1|A_1|+[(|A_2|-1)\cdot 1+  2]\cdot W_2+1\cdot W_3 |A_3|\\
& = n+ (3n+1)(4|E|+n)+(3n+1)+ n\\& = (3n+1)(4|E|+n)+5n+1\stackrel{\eqref{alpha}}{>}\alpha
\end{align*}
a contradiction.
\end{proof}
Essentially, by choosing $W_2$ to be large, we enforce that all ``demands'' in $A_2$ are satisfied by a direct edge in $\myset{S}$. The next lemma shows a similar result for $A_1$. Using shortcut edges to satisfy these ``demands'' is enforced by making the distance $\ell_1$ very large.
\begin{lemma}\label{lemmaS1}
For every $i\in V$, there exists at least one shortcut edge in $\myset{S}$ whose origin is in the same row as $a_i$ and in a column to the left of $b_i$. Moreover, this edge is used during the greedy forwarding of a message from $a_i$ to $b_i$.
\end{lemma}
\begin{proof}
Suppose not. Then, there exists an $i\in V$ such that no shortcut edge has its origin  between $a_i$ and $b_i$, or such an edge exists but is not used by the greedy forwarding from $a_i$ to $b_i$ (\emph{e.g.}, because it points too far from $b_i$). Then, the greedy forwarding from $a_i$ to $b_i$ will use only local edges and, hence, $$C_{\mathcal{S}}(a_i,b_i)=\ell_1.$$
We thus have that
\begin{align*}
\bar{C}^w_\myset{S} &\geq  W_1[|A_1|-1+\ell_1]+W_2|A_2|+W_3|A_3| \\&= \ell_1+2n-1+W_2|A_2|.\\
&\stackrel{\eqref{l1}}{=}6n^2+5n+1+W_2|A_2|
\end{align*}
On the other hand, by \eqref{alpha}
$$\alpha = 5n+ W_2|A_2|$$
so $\bar{C}^w_\myset{S}>\alpha$, a contradiction.
\end{proof}
Let $S_1$ be the set of all edges whose origin is between some $a_i$ and $b_i$, $i\in V$, and that are used during forwarding from this $a_i$ to $b_i$. Note that Lemma~\ref{lemmaS1} implies that $|S_1|\geq n$.
\begin{lemma}\label{lemmaL1} The target of any edge in $S_1$ must lie to the left of the $2\ell_1+1$-th column of the grid
\end{lemma}
\begin{proof}
The Manhattan distance of $a_i$ to $b_i$ is $\ell_1$, so its left local neighbor lies at $\ell_1-1$ steps from $b_i$. Greedy forwarding is monotone, so the Manhattan distance from $b_i$ of any target of an edge followed subsequently to route towards $b_i$ must  be less than $\ell_1$. 
\end{proof}
Essentially, all edges in $S_1$ must point close enough to $b_i$, otherwise they would not be used in greedy forwarding. This implies that, to forward the ``demands'' in $A_3$, that connect the leftmost to the rightmost nodes on the grid, an \emph{additional} set of shortcut edges, that are neither in $S_1$ nor in $A_2$, need to be used.
\begin{lemma}\label{lemmaL3} For every $i\in V$, there exists at least one shortcut edge in $\myset{S}$ that is used when forwarding a message from $a_i$ to $d_i$ that is neither in $S_1$ nor in $A_2$.
\end{lemma}
\begin{proof}
Suppose not. By Lemma~\ref{lemmaL1}, the target of any edge in $S_1$ is to the left of the $2\ell_1+1$ column. Recall that
$$ A_2 = \{(b_i,b_j)\mid (i,j)\in E \}\cup \{(c_i,d_j)\mid (i,j)\in E\}\cup\{(c_i,d_i)\mid i\in V\}$$
By the definition of $b_i$, $i \in V$, the targets of the edges in $\{(b_i,b_j)\mid (i,j)\in E \}$ lie on the $(\ell_1+1)$-th column. Similarly, the origins of the edges in $\{(c_i,d_j)\mid (i,j)\in E\}\cup\{(c_i,d_i)\mid i\in V\}$ lie on the $\ell_1+\ell_2+1$-th column.

As a result, if the lemma does not hold, there is a demand in $A_3$, say $(a_i,d_i)$, that does not use any additional shortcut edges. This means that the distance between the $2\ell+1$ and the  $\ell_1+\ell_2+1$-th column is traversed by using local edges. Hence, 
$$C_{\mathcal{S}}(a_i,d_i)\geq \ell_2-\ell_1+1 $$
as at least one additional step is needed to get to the $2\ell_1+1$-th column from $a_i$.
This implies that 
\begin{align*}
\bar{C}_{\mathcal{S}}^w &\geq W_1|A_1|+W_2|A_2|+W_3[|A_3|-1]+W_3(\ell_2-\ell_1+1) \\
&=2n+W_2|A_2|+\ell_2-\ell_1\stackrel{\eqref{l2}}{=}  W_2|A_2|+5n+1>\alpha
\end{align*}
a contradiction.
\end{proof}
Let $S_3=\myset{S}\setminus(S_1\cup A_2)$. Lemma~\ref{lemmaL3} implies that $S_3$ is non-empty, while Lemmas \ref{lemmaS2} and \ref{lemmaS1}, along with the fact that $|\myset{S}|\leq\beta= |A_2|+n+k$, imply that $|S_3|\leq k$. The following lemma states that some of these edges must have targets that are close enough to the destinations $d_i$.
\begin{lemma}\label{lemmafromdest} For each $i\in V$, there exists an edge in $S_3$ whose target is within Manhattan distance $3n+1$ of either $d_i$ or $c_j$, where $(c_j,d_i)\in A_2$. Moreover, this edge is used for forwarding a message from $a_i$ to $d_i$ with greedy forwarding.
\end{lemma}
\begin{proof}
Suppose not. Then there exists an $i$ for which greedy forwarding from $a_i$ to $d_i$ does not employ any edge fitting the description in the lemma. 
Then, the destination $d_i$  can not be reached by a shortcut edge in either $S_3$ or $A_1$ whose target is closer than $3n+1$ steps. Thus, $d_i$ is reached in one of the two following ways: either  $3n+1$ steps are required in reaching it, through forwarding over local edges, or an edge $(c_j,d_i)$ in $A_2$ is used to reach it. In the latter case,  reaching $c_i$ also requires at least $3n+1$ steps of local forwarding, as no edge in $A_2$ or $S_3$ has an target within $3n$ steps from it, and any edge in $S_1$ that may be this close is not used (by the hypothesis).
As a result,
$$C_{\mathcal{S}}(a_i,d_i)\geq 3n+2 $$
as at least one additional step is required in reaching the ball of radius $3n$ centered around $d_i$ or $c_i$ from $a_i$.
This gives us
\begin{align*}\bar{C}_{\mathcal{S}}^w &\geq W_1|A_1|+W_2|A_2|+W_3(|A_3|-1)+W_3\cdot (3n+2) \\
&= 5n + W_2|A_2|+1> \alpha
 \end{align*}
a contradiction.
\end{proof}
When forwarding from $a_i$ to $d_i$, $i \in V$, there may be more than one edges in $S_3$ fitting the description in Lemma~\ref{lemmafromdest}. For each $i\in V$, consider the \emph{last} of all these edges. Denote the resulting subset by $S_3'$ ---note that, by definition $|S_3'|\leq |S_3|\leq k$. 

For each $i$, there exists \emph{exactly one} edge in $S_3'$ that is used to forward a message from $a_i$ to $d_i$. 
%Thus, the set $V$ can be partitioned in two $k'$ subsets $V_1,\ldots,V_k'$, where $k'\leq k$ and $i$ and $j$ belong to the same partition if the same edge in $S_3'$  is used when forwarding from $a_i$ to $d_i$ and from $a_j$ to $d_j$.
Moreover, recall that $\ell_0=\ell_3=6n+3$. Therefore, the Manhattan distance between any two nodes in $\{c_1,\ldots,c_n\}\cup\{d_1,\ldots,d_n\}$ is $2 (3n+1)+1$. As a result, the targets of the edges in $S_3'$ will be within distance $3n+1$ of \emph{exactly one} of the nodes in the above set. 

Let $A\subset V$ be the set of all vertices $i\in V$ such that the unique edge in $S_3'$ used in forwarding from $a_i$ to $d_i$ has an target within distance $3n+1$ of either $c_i$ or $d_i$. Then $A$ is a vertex cover of $G$, and $|A|\leq k$. To begin with,  $|A|\leq k$ because each target of an edge in $S_3'$ can be within distance $3n+1$ of only one of the nodes in $\{c_1,\ldots,c_n\}\cup\{d_1,\ldots,d_n\}$, and there are at most $k$ edges in $S_3'$.

To see that it covers the graph $G$, suppose that $j\in V\setminus A$. Then, by Lemma~\ref{lemmafromdest}, the edge in $S_3'$ corresponding to $i$ is either pointing within distance $3n+1$ of either $d_j$ or a $c_i$ such that $(c_i,d_j)\in A_2$. By the construction of $A$, it cannot point in the proximity of $d_j$, because then $j\in A$, a contradiction. Similarly, it cannot point in the proximity of $c_j$, because then, again, $j\in A$, a contradiction. Therefore, it points in the proximity of some $c_i$, where $i\neq j$ and $(c_i,d_j)\in A_2$. By the construction of $A$, $i\in A$. Moreover, by the definition of $A_2$, $(c_i,d_j)\in A_2$ if and only if $(i,j)\in E$. Therefore, $j\in \Gamma(A)$. As $j$ was arbitrary, $A$ is a vertex cover of $G$. 
\end{proof}
\begin{comment}
{\em\small A few observations: 
\begin{itemize}
\item In the above construction, $\beta=\bigO{n^2}$ and  $|A_1\cup A_2 \cup A_3|=\bigO{n^2}$. Given that $N=\bigT{n^4}$, the above imply that the general problem remains $NP$-hard if it is restricted either of the following cases:
\begin{itemize}
\item The support of $\lambda(i,j)$ is $\bigO{\sqrt{N}}$, or
\item $\beta= \bigO{\sqrt{N}}$.
\end{itemize}
A negative aspect of the above observation is that NP-hardness is not implied when $\beta=\bigOm{N}$, which is the case of interest if, \emph{e.g.}, one is to assume that each node has at least one shortcut edge.
\item The proof obviously extends as is to any $d$-dimensional grid, where $d>2$. Interestingly, an almost identical proof can be used to show NP-hardness for a grid of dimension $d=1$ (a single row). In particular, each of the four columns of points $a_\cdot$, $b_\cdot$, $c_\cdot$, and $d_\cdot$ can be placed sequentially on a single row. By taking the distances between any two consequtive points to be large enough, we can guarantee that all the lemmas made in the proof of the $d=2$ case still hold.
%\item I believe that the proof can be modified to show the problem is not only NP-hard, but also that no polynomial time algorithm  acheives a constant approximation factor unless $P=NP$. The idea is to make the distances between nodes large enough so that, if a vertex cover does not exist, the aggregate cost will become arbitrarily large.
\end{itemize}
}

\end{comment}


==> learning_short.tex <==
\section{Learning Algorithm}\label{section:learning}
\begin{comment}
Section~\ref{section:mainresults} established bounds on the cost of greedy content search provided that the  distribution \eqref{shortcutdistr} is used to propose items to the oracle. Hence, if the  embedding of $\myset{N}$ in $(\myset{M},d)$ and target distribution $\mu$  are known, it is possible to perform greedy content search with the performance guarantees provided by Theorem~\ref{th:content-search}.
\end{comment}
 In this section, we turn our attention to how such bounds can be achieved if \emph{neither} the  embedding in $(\myset{M},d)$ \emph{nor} the target distribution $\mu$ are a priori known. To this end, we propose a novel adaptive algorithm that achieves the performance guarantees of  Theorem~\ref{th:content-search} without access to the above information.

Our algorithm effectively learns the ranks $r_x(y)$ of objects and the target distribution $\mu$ as time progresses. %st, it requires no a priori knowledge of the distances of objects in the metric space $(\myset{M},d)$. Instead, 
It does not require that distances between objects are at any point disclosed; instead, we assume that it only has access to a comparison oracle. 

%slightly stronger than the one described in Section~\ref{section:smallworld}. %For this reason, our mechanism also works even if objects are not embedded 

It is important to note that our algorithm is \emph{adaptive}: 
%though we prove its convergence under a stationary regime, the algorithm can operate in a dynamic environment.
for example, new objects can be added to the database while old ones can be removed. Moreover, the popularity of objects can change as time progresses. Provided that such changes happen infrequently, at a larger timescale compared to the timescale in which database queries are submitted, our algorithm will be able to adapt and  converge to the desired behavior.
%Moreover, both the learning and the proposals made by our algorithm can be implemented in a distributed manner. In particular, each object maintains a set of local variables, that can be updated through message exchanges between objects. A query for a target object can be forwarded from one object to the next, and the forwarding decision is determined locally at each object, through greedy content search. As a result, the mechanism can operate in a distributed databases, where different objects can be stored at different machines.

%\subsection{Demand Model}
\subsubsection{Demand Model and Probabilistic Oracle:}
We  assume that time is slotted and that at each timeslot $\tau=0,1,\ldots$ a new query is generated in the database.
\begin{comment}
 As before, we assume that the source and target of the new query are selected according to a demand distribution $\lambda$ over $\Nn\times \Nn$. We again denote by $\nu$, $\mu$ the (marginal) source and target distributions, respectively. 
\end{comment}
Our algorithm will require that the support of both the source and target distributions is $\Nn$, and more precisely that $\lambda(x,y)>0,$ for all $x,y\in \Nn$.
%\begin{align}\label{strong}\lambda(x,y)>0, \text{ for all }x,y\in \Nn.\end{align}
The requirement that the target set $\myset{T}=\supp(\mu)$  is $\Nn$ is necessary to ensure learning; we can only infer the relative order w.r.t.~objects $t$ for which questions of the form $\oracle(x,y,t)$ are submitted to the oracle.
Moreover, it  is natural in our model to assume that the source distribution $\nu$ is at the discretion of our algorithm: we can choose which objects to propose first to the user/oracle.
\begin{comment}
 In this sense, for a given target distribution $\mu$ s.t.~$\supp(\mu)=\Nn$, \eqref{strong} can be enforced, \emph{e.g.}, by selecting source objects uniformly at random from $\Nn$ and independently of the target. 
 \end{comment}
 %In this section, we will assume that the source distribution $\nu$ is at the discretion of the algorithm: the algorithm can choose which object to show to the user. In particular, we assume that the source distribution is uniform and independent of the target distribution $\mu$.

We consider a slightly stronger oracle than the one described in Section~\ref{section:contentsearch}.  In particular, we again assume that
\begin{comment}
 In particular, we again assume that
\begin{equation}
\text{\oracle}(x,y,t)=\left\{
\begin{array}{ll} 
x & \text{if } x\lst{t} y,\\ 
y & \text{if } x\grt{t} y.
\end{array} \right.
\end{equation}
However, we further assume that 
\end{comment}
if $x\eqvl{t}y$, then $\oracle(x,y,t)$ can return either of the two possible outcomes \emph{with non-zero probability}. This is stronger than the oracle in  Section~\ref{section:contentsearch}, where we assumed that the outcome will be arbitrary. %Keeping in mind that the oracle models the behavior of human users, the above behavior states that humans sometimes select $x$ and sometimes select $y$ as the object closest to $t$, and both outcomes has some likelihood (not necessarily equal) of being returned. 
\begin{comment}
We should point out here that this is still weaker than an oracle that correctly identifies  $x\eqvl{t} y$ (\emph{i.e.}, the human states that these objects are at equal distance from $t$) as, given such an oracle, we can implement the above probabilistic oracle by simply returning $x$ or $y$ with equal probability.
\end{comment}
%In our scenario, it is more natural to assume that the source distribution (\emph{i.e.}, the first item from which the greedy content search starts) is left to the discretion of the algorithm. In particular, as we will see, our convergence result (Theorem~\ref{convergence}) requires that $\supp(\mu)\subseteq \supp(\nu)$. To achieve this, the algorithm can trivially start from an object selected uniformly at random from $\Nn$, independently of the target.



\subsubsection{Data Structures:}
For every object $x\in\Nn$, the database storing $x$ also maintains the following associated data structures. The first data structure is a counter keeping track of how often the object $x$ has been requested so far. The second data structure maintains an order of the objects in $\Nn$; at any point in time, this total order is an ``estimator'' of $\lsteq{x}$, the order of objects with respect to their distance from $x$. We describe each one of these two data structures in more detail below.

\paragraph{Estimating the Target Distribution:}

The first data structure associated with an object $x$ is an estimator of $\mu(x)$, \emph{i.e.}, the probability with which $x$ is selected as a target. A simple method for keeping track of this information is through a counter $C_x$. This counter $C_x$ is initially set to zero and is incremented every time  object $x$ is the target. If $C_x(\tau)$ is the counter at timeslot $\tau$, then $\hat{\mu}(x) =C_x(\tau)/\tau$
% \begin{align}\hat{\mu}(x) =C_x(\tau)/\tau \label{muest}\end{align}
is  an "unbiased estimator" of $\mu(x)$. To avoid counting to infinity %, but also to address cases in which the distribution $\mu$ is not stationary 
a ``moving average'' (\emph{e.g.}, and exponentially weighted moving average) could be used instead.


\paragraph{Maintaining a Partial Order:}
The second data structure $\myset{O}_x$ associated with each $x\in\Nn$ maintains a total order of objects in $\Nn$ w.r.t.~their similarity to $x$. 
It supports an operation called \order() that returns a partition of objects in $\Nn$ along with a total order over this partition. In particular, the output of $\myset{O}_x.\order()$ consists of an ordered sequence of disjoint sets $A_1, A_2,\ldots, A_j$, where $\bigcup A_i=\Nn\setminus\{x\}$. Intuitively, any two objects in a set $A_i$ are considered to be at equal distance from $x$, while among two objects $u\in A_i$ and $v\in A_j$ with $i<j$ the object $u$ is assumed to be the closer to $x$.

\sloppy
Moreover, every time that the algorithm evokes $\oracle(u,v,x)$, and learns, \emph{e.g.}, that $u\lsteq{x} v$, the data structure $\myset{O}_x$ should be updated to reflect this information. In particular, if the algorithm has learned so far the order relationships \begin{align}u_1\lsteq{x} v_1,\quad u_2\lsteq{x} v_2,\quad \ldots, \quad u_i\lsteq{x} v_i\label{learnedorder}\end{align}
 $\myset{O}_x$.\order() should return the objects in $\Nn$ sorted in such a way that all relationships in \eqref{learnedorder} are respected. In particular, object $u_1$ should appear before $v_1$, $u_2$ before $v_2$, and so forth. To that effect, the data structure should also support an operation called $\myset{O}_x$.\add($u$,$v$) that adds the order relationship $u \lsteq{x} v$ to the constraints respected by the output of $\myset{O}_x$.\order().
\fussy
\begin{comment}
A simple (but not the most efficient) way of implementing this data structure is to represent order relationships through a directed acyclic graph. Initially, the graph's vertex set is $\Nn$ and its edge set is empty. Every time an operation \add($u$,$v$)  is executed, an edge is added between vertices $u$ and $v$. If the addition of the new edge creates a cycle then all nodes in the cycle are collapsed to a single node, keeping thus the graph acyclic. Note that the creation of a cycle $u\to v\to\ldots\to w\to u$ implies that $u\eqvl{x}v\eqvl{x}\ldots\eqvl{x}w$, \emph{i.e.}, all these nodes are at equal distance from $x$. 

Cycles can be detected by using depth-first search over the DAG \cite{clrs}. The sets $A_i$ returned by \order\ are the sets associated with each collapsed node, while a total order among them that respects the constraints implied by the edges in the DAG can be obtained either by depth-first search or by a topological sort \cite{clrs}. Hence, the \add()  and \order() operations have a worst case cost of $\Theta(n+m)$, where $m$ is the total number of edges in the graph. 

Several more efficient algorithms exist in literature \cite{tarjanfast,pearce,bender}, the best \cite{bender} yielding a cost of $O(n)$ for \order\ and an aggregate cost of at most $O(n^2\log n)$ for any sequence of \add\ operations. We stress here  that any of these   implementations could be used for our purposes. We refer the reader interested in such implementations to  \cite{tarjanfast,pearce,bender} and, to avoid any ambiguity, we assume the above na\"ive approach for the remainder of this work.
\end{comment}
Several  efficient algorithms exist in literature \cite{tarjanfast,pearce,bender}, the best \cite{bender} yielding a cost of $O(n)$ for \order\ and an aggregate cost of at most $O(n^2\log n)$ for any sequence of \add\ operations. We stress here  that any of these more efficient implementations could be used for our purposes. 

\subsubsection{Greedy Content Search:}
Our learning algorithm implements greedy content search, as described in Section~\ref{section:contentsearch}, in the following manner. When a new query is submitted to the database, the algorithm first selects a source $s$ uniformly at random. It then performs greedy content search 
using a memoryless selection policy $\hat{\myset{F}}$ with distribution $\hat{\ell}_{x}$, \emph{i.e.}, $\Pr(\hat{\myset{F}}(\myset{H}_k,x_k) = w)=\hat{\ell}_{x_k}(w)$ for $w\in\Nn.$
%\begin{align}\Pr(\myset{F}(\myset{H}_k,x_k) = w)=\hat{\ell}_{x_k}(w)\quad w\in\Nn. \label{hatpolicy}\end{align}
Below, we discuss in detail how  $\hat{\ell}_{x}$, $x\in\Nn$, are computed. 

 When the current object $x_k$, $k=0,1,\ldots$, is equal to $x$, the algorithm evokes $\myset{O}_{x_k}$.\order() and obtains an ordered partition $A_1,A_2,\ldots,A_{j}$ of items in $\Nn\setminus\{x\}$. We define $\hat{r}_x(w)=\sum_{j=1}^{i:w\in A_i} \hat{\mu}(A_j),$ for $w\in \Nn\setminus\{x\}.$
 %$$\hat{r}_x(w)=\sum_{j=1}^{i:w\in A_i} \hat{\mu}(A_j), \quad w\in \Nn\setminus\{x\}.$$
This can be seen as an ``estimator'' of the true rank $r_x$ given by \eqref{rank}. The distribution $\hat{\ell}_{x}$ is then computed as follows:
\begin{align}\hat{\ell}_x(w) = \frac{\hat{\mu}(w)}{\hat{r}_x(w)}\frac{1-\epsilon}{\hat{Z}_x}+ \frac{\epsilon}{n-1},\quad i=1,\ldots,n-1, \label{hatell}\end{align}
where $\hat{Z}_x=\sum_{w\in \Nn\setminus\{x\}} \hat{\mu}(w)/\hat{r}_x(w)$ is a normalization factor and $\epsilon>0$ is a small constant.
An alternative view of \eqref{hatell} is that the object proposed is selected uniformly at random with probability $\epsilon$, and proportionally to $\hat{\mu}(w_i)/\hat{r}_x(w_i)$ with probability $1-\epsilon$. The use of $\epsilon>0$ guarantees that every search eventually finds the target $t$. 

Upon locating a target $t$, any access to the oracle in the history $\history_k$ can be used to update  $\myset{O}_t$; in particular, a call \oracle($u$,$v$,$t$) that returns $u$ implies the constraint $u\lsteq{t} v$, which should be added to the data structure through $\myset{O}_t$.\add($u,v$). Note that this operation can take place only at the \emph{end of the greedy content search}; the outcomes of calls to the oracle can be observed, but the target $t$ is  revealed only after it has been located.

Our main result is that, as $\tau$ tends to infinity, the above algorithm achieves performance guarantees arbitrarily close to the ones of Theorem~\ref{th:content-search}.

Let $\hat{\myset{F}}(\tau)$ be the selection policy as defined above at timeslot $\tau$ and denote by $\bar{C}(\tau)$
%$$\bar{C}(\tau) = \sum_{(s,t\in \Nn\times \Nn}\lambda(s,t)\sum_{s\in \Nn} \expect[C_{\hat{F}(\tau)}(s,t)] $$
the expected search cost at timeslot $\tau$. Then the following theorem holds:
\begin{theorem}\label{convergence}
Assume that for any two targets $u,v\in\Nn$, $\lambda(u,v)>0$.
$$\limsup_{\tau\to\infty}\bar{C}(\tau)\leq \frac{6 c^3(\mu) H(\mu) H_{\max}(\mu)}{(1-\epsilon)}.$$
\begin{comment}
where $c(\mu)$, $H(\mu)$ and $H_{\max}(\mu)$ are the doubling parameter, the entropy and the max entropy, respectively, of the target distribution $\mu$.
\end{comment}
\end{theorem}

%\section{Proof of Theorem~\protect\lowercase{\ref{convergence}}}\label{proofofconvergence}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{proof} 
Let $\Delta_\mu= \sup_{x\in \Nn} |\hat{\mu}(x)-\mu(x)|$.
Observe first that, by the weak law of large numbers, for any $\delta>0$
\begin{align}\label{weak}\lim_{\tau\to\infty} \Pr(\Delta_\mu>\delta)=0.\end{align}
\emph{i.e.}, $\hat{\mu}$ converges to $\mu$ in probability.
The lemma below states, for every $t\in \Nn$, the  order data structure $\myset{O}_t$ will learn the correct order of any two objects $u,v$ in finite time. 
\begin{lemma}\label{learnorder}
Consider $u,v,t\in\myset{N}$ such that $u\lsteq{t} v$. Then, the order data structure in $t$ evokes $\myset{O}_t$.\emph{\add}($u$,$v$) after a finite time, with probability one.
\end{lemma}
\begin{proof}
Recall that $\myset{O}_t$.\emph{\add}($u$,$v$) is evoked if and only if a call $\oracle(u,v,t)$ takes place and it returns $u$. If $u\lst{t} v$ then $\oracle(u,v,t)=u$. If, on the other hand, $u\eqvl{t}v$, then $\oracle(u,v,t)$ returns $u$ with non-zero probability. It thus suffices to show that such, for large enough $\tau$, a call $\oracle(u,v,t)$ occurs at timeslot $\tau$ with a non-zero probability. 
By the  hypothesis of Theorem~\ref{convergence}, $\lambda(u,t)>0$. By \eqref{hatell}, given that the source is $u$, the probability that $\hat{\myset{F}}(u)=v$ conditioned on $\hat{\mu}$  is
\begin{align*}\hat{\ell}_u(v)& \geq \frac{\mu(v)\!-\!\Delta_\mu}{1\!+\!(n\!-\!1)\Delta_\mu}\frac{1\!-\!\epsilon}{n\!-\!1}\!+\!\frac{\epsilon}{n\!-\!1}\geq \frac{\mu(v)\!-\!\Delta_\mu}{(1\!+\!(n\!-\!1)\Delta_\mu)(n\!-\!1)}\end{align*}
as $\hat{Z}_v\leq n-1$ and $|\hat{\mu}(x)-\mu(x)|\leq \Delta_\mu$ for every $x\in \Nn$.
 Thus, for any $\delta>0$, the probability that  is lower-bounded by $$\lambda(u,t)\Pr(\hat{\myset{F}}(u)=v)\geq \frac{\mu(v)-\delta}{1+(n-1)\delta}\Pr(\Delta_\mu<\delta).$$
By taking $\delta>0$ smaller than $\mu(v)$, we have by \eqref{weak} that there exists a $\tau^*$ s.t.~for all $\tau>\tau^*$ the probability that $\oracle(u,v,t)$ takes place at timeslot $\tau$ is bounded away from zero, and the lemma follows.
%$\lambda(u,t)\Pr(\hat{\myset{F}}(u)=v)\geq \frac{\mu(v)-\delta}{1+(n-1)\delta}\Pr(\Delta_\mu<\delta)$ by from 0 for sufficiently small $\delta$. On the other hand, by \eqref{weak}, there exists a $\tau^*$ such that for all $\tau>\tau*$ 
\end{proof}
\sloppy Thus if $t$ is a target then, after a finite time, for any two $u,v\in \Nn$ the ordered partition $A_1,\ldots,A_j$ returned by $\myset{O}_t.\order()$ will respect the relationship between $u,v$. In particular for $u\in A_i$,$v\in A_{i'}$, if $u\eqvl{t}v$ then $i=i'$, while if $u\lst{t}v$ then $i<i'$. As a result, the estimated rank of an object $u\in A_i$ w.r.t.~$t$ will satisfy
$$\hat{r}_t(u)=\!\!\!\!\sum_{x\in \myset{T}: x\lst{v} u}\!\!\!\!\hat{\mu}(x)+\!\!\!\!\sum_{x\in\Nn\setminus\myset{T}:x\in A_{i'},i'\leq i}\!\!\!\!\hat{\mu}(x) =r_t(u)+O(\Delta_\mu)$$
\emph{i.e.} the estimated rank will be close to the true rank, provided that $\Delta_\mu$ is small. Moreover, as in Lemma~\ref{normalization}, it can be shown that  $$\hat{Z}_v \leq 1\!+\!\log^{-1} \hat{\mu}(v)=1\!+\!\log^{-1} [\mu_v+O(\Delta_\mu)]$$ for $v\in \myset{N}$. From these, for $\Delta_\mu$ small enough,
we have that for $u,v\in \myset{N}$, 
$$\hat{\ell}_u(v) = [\ell_u(v)+O(\Delta_\mu)](1-\epsilon)+ \epsilon \frac{1}{n-1}.$$
Following the same steps as the proof of Theorem~\ref{th:small-world} we can show that, given that $\Delta_\mu\leq \delta$, the expected search cost is upper bounded by
$\frac{6c^3HH_{\max}}{(1-\epsilon) +O(\delta)}$. This gives us that
$$\bar{C}(\tau) \leq \Big[\frac{6c^3HH_{\max}}{(1-\epsilon)} +O(\delta)\Big]\Pr(\Delta_\mu\leq \delta)+ \frac{n-1}{\epsilon} \Pr(\Delta_\mu>\delta) $$
where the second part follows from the fact that, by using the uniform distribution with probability $\epsilon$, we ensure that the cost is stochastically upper-bounded by a geometric r.v.~with parameter $\frac{\epsilon}{n-1}$. Thus, by \eqref{weak}, % for small enough $\delta>0$.
$$\limsup_{\tau\to\infty} \bar{C}(\tau)\leq \frac{6c^3HH_{\max}}{(1-\epsilon)} +O(\delta). $$
As this is true for all small enough delta, the theorem follows.\hspace*{\stretch{1}}\qed
%On the other hand, the same cannot be said for $\hat{\ell}_u$ when $u\notin \myset{T}$: in effect the data structure $\myset{O}_u$ is never updated, as it is not a target. However, irrespectively of ranks, as the estimated target probabilities of non-targets are small, there will be a high probability that, when at a non-target $u$, the next node proposed will in fact be a target. 


\fussy
\end{proof}
\end{comment}
%The proof of this theorem can be found in Appendix~\ref{proofofconvergence}.
\begin{comment}
\subsection{Extensions}
To do:
\begin{itemize}
\item Distributed version.
\item Dynamic/adaptive: we can add/remove objects easily.
\end{itemize}
\end{comment}

